NetTiSA: Extended IP Flow with Time-series Features for Universal Bandwidth-constrained High-speed Network Traffic Classification

Network traffic monitoring based on IP Flows is a standard monitoring approach that can be deployed to various network infrastructures, even the large IPS-based networks connecting millions of people. Since flow records traditionally contain only limited information (addresses, transport ports, and amount of exchanged data), they are also commonly extended for additional features that enable network traffic analysis with high accuracy. Nevertheless, the flow extensions are often too large or hard to compute, which limits their deployment only to smaller-sized networks. This paper proposes a novel extended IP flow called NetTiSA (Network Time Series Analysed), which is based on the analysis of the time series of packet sizes. By thoroughly testing 25 different network classification tasks, we show the broad applicability and high usability of NetTiSA, which often outperforms the best-performing related works. For practical deployment, we also consider the sizes of flows extended for NetTiSA and evaluate the performance impacts of its computation in the flow exporter. The novel feature set proved universal and deployable to high-speed ISP networks with 100\,Gbps lines; thus, it enables accurate and widespread network security protection.

==> table_binary_results_old.tex <==

        \begin{table*}
        % \begin{minipage}{.59\linewidth}
            \caption{Final results (in \%) of the testing phase of binary classification based on the NetTiSA flow}
            % . Results contain achieved scores of the best model from the validation phase on the test dataset, and they are compared with the best results from related works. Furthermore, the table contains the results of K-Fold validation with 10 folds. However, most related works do not present the results of K-fold validation.
            \begin{center}
                \begin{tabular}{|Q|Q|Y|Z{1.5cm}|Z{1.5cm}|Z{1.5cm}|Z{1.5cm}|}
                    \hline 
                    \rowcolor{Gray} \textbf{Detection problem} &  \textbf{Method} & \textbf{} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
                    \hline
                    
                    \rowcolor{white}   &  & Test & 99.85 & 99.91 & \textbf{99.89} & 99.90 \\
                    & \multirow{-2}{*}{Stergiopoulos  et  al.   \cite{stergiopoulos2018automatic}}  & KFold & -- & -- & -- & -- \\
                    \cline{2-7}
                    \rowcolor{white} &  & Test & \textbf{99.98} & \textbf{100.0} & 99.86 & \textbf{99.93} \\
                     &  &  & \textbf{99.88} & \textbf{99.81}  & \textbf{99.53} & \textbf{99.67}  \\
                    \multirow{-5}{*}{\textbf{Botnet}} & \multirow{-3}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & \textbf{(\(\pm\) 0.052)} & \textbf{(\(\pm\) 0.201)} & \textbf{(\(\pm\) 0.156)} & \textbf{(\(\pm\) 0.131)} \\
                    \hline
                    
                    \rowcolor{white}   &  & Test &  93.72 & \textbf{99.99} & 82.81 & 90.59 \\
                    & \multirow{-2}{*}{Plný et  al.   \cite{plny2023decrypto}}  & KFold & -- & -- & -- & -- \\
                    \cline{2-7}
                    \rowcolor{white} &  & Test & \textbf{99.35} & 99.62 & \textbf{98.60} & \textbf{99.10} \\
                    & & & \textbf{99.27} & \textbf{99.59} & \textbf{98.41} & \textbf{99.00} \\
                    \multirow{-5}{*}{\textbf{Cryptomining}} & \multirow{-3}{*}{NetTiSA} & \multirow{-2}{*}{KFold} &  \textbf{(\(\pm\) 0.029)} & \textbf{(\(\pm\) 0.027)} &  \textbf{(\(\pm\) 0.071)} &  \textbf{(\(\pm\) 0.040)} \\
                    \hline
                    \rowcolor{white}   &  & Test &  &  &  &  \\
                    \cline{2-7}
                    \multirow{-2}{*}{\textbf{DoH - CIC}} & NetTiSA & Test & 99.90 & 99.89 & 99.77 & 99.83 \\
                    \hline
                    \rowcolor{white} &  & Test & \textbf{97.79} & \textbf{97.81} & \textbf{99.81} & \textbf{98.80} \\
                     & & & \textbf{97.95} & \textbf{97.97} & \textbf{99.84} & \textbf{98.89} \\
                    \multirow{-3}{*}{\textbf{DoH - Real-world}} & \multirow{-3}{*}{NetTiSA}  & \multirow{-2}{*}{KFold} &  \textbf{(\(\pm\) 0.024)} & \textbf{ (\(\pm\) 0.022)} &  \textbf{(\(\pm\) 0.013)} & \textbf{(\(\pm\) 0.015)} \\
                    \hline
                    
                    \rowcolor{white} &  & Test & 99.99  & 99.99 & 99.99 & 99.99 \\
                     & \multirow{-3}{*}{Shagiq et al. \cite{SHAFIQ2020433}} & KFold & 99.99(\(\pm\)-) & 99.99(\(\pm\)-) & 99.99(\(\pm\)-) & 99.99(\(\pm\)-) \\
                    \cline{2-7}
                    \rowcolor{white} &  & Test &  \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} \\
                    & & & \textbf{100.0} & \textbf{99.99}  & \textbf{100.0} & \textbf{99.99}  \\
                    \multirow{-6}{*}{\textbf{(D)DoS}} & \multirow{-3}{*}{NetTiSA} & \multirow{-2}{*}{KFold} &  \textbf{(\(\pm\) 0.0)} &  \textbf{(\(\pm\) 0.012)} &  \textbf{(\(\pm\) 0.0)} &  \textbf{(\(\pm\) 0.006)} \\
                    \hline
                    \rowcolor{white} &  & Test &  $\thicksim 96$ & $\thicksim 95$ & $\thicksim 97$ &  $\thicksim 96$ \\ 
                    % & &  &   &  &  &  \\ 
                     & \multirow{-2}{*}{ Sahu et al. \cite{sahu2021internet}  } & \multirow{-1}{*}{KFold} & -- & -- & -- & -- \\ 
                     
                     % (\(\pm\) )  & (\(\pm\) )  & (\(\pm\) ) &  (\(\pm\) )  \\ 
                    \cline{2-7}
                    \rowcolor{white} &  & Test & \textbf{99.86} & \textbf{99.95} & \textbf{99.87} & \textbf{99.91} \\
                    & & & \textbf{99.86} & \textbf{99.95} & \textbf{99.86} & \textbf{99.90} \\
                    \multirow{-6}{*}{\textbf{IoT Malware}} & \multirow{-3}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & \textbf{(\(\pm\) 0.006)} & \textbf{(\(\pm\) 0.003)}  & \textbf{(\(\pm\) 0.009)} & \textbf{(\(\pm\) 0.004)} \\
                    \hline
                    \rowcolor{white} &  & Test & 99.19  & 99.22 & 99.19 & 99.20  \\
                    & &  & 99.19  & 99.22 & \textbf{99.19} & \textbf{99.20} \\ 
                     & \multirow{-3}{*}{Kumaar et al. \cite{kumaar2021hybrid}  } & \multirow{-2}{*}{KFold} & (\(\pm\) 0.015)  & (\(\pm\) 0.015) & \textbf{(\(\pm\) 0.015)} &  \textbf{(\(\pm\) 0.015)} \\ 
                    \cline{2-7}
                    \rowcolor{white} &  & Test & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} \\
                    & & & \textbf{99.85} & \textbf{100.0} & 96.0 & 97.93 \\
                    \multirow{-6}{*}{\textbf{Malware DNS}} & \multirow{-3}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & \textbf{(\(\pm\) 0.150)} & \textbf{(\(\pm\) 0.0)} & (\(\pm\) 3.741) & (\(\pm\) 1.968) \\
                    \hline
                    
                    \rowcolor{white} &   & Test & 99.89 & 99.88 & \textbf{99.89}  & \textbf{99.88}  \\ 
                     &  \multirow{-2}{*}{Sarkar et al. \cite{sarkar2020detection}}  & KFold & -- & -- & -- & -- \\ 
                    \cline{2-7}
                    \rowcolor{white} &  & Test &  \textbf{99.98} & \textbf{100.0} & 99.25 & 99.62 \\
                    & & & \textbf{99.93} & \textbf{99.62} & \textbf{96.75} & \textbf{98.14} \\
                    \multirow{-5}{*}{\textbf{TOR}} & \multirow{-3}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & \textbf{(\(\pm\) 0.056)} &  \textbf{(\(\pm\) 0.578)} & \textbf{(\(\pm\) 2.143)} & \textbf{(\(\pm\) 1.229)} \\
                    \hline
                    
                    \rowcolor{white} &   & Test  & \textbf{97.20} & \textbf{96.98} & 96.42 & \textbf{96.63}  \\
                     & \multirow{-2}{*}{Sun et al. \cite{sun2023deep}}  & KFold & -- & -- & -- & -- \\
                    \cline{2-7}
                    \rowcolor{white} &  & Test &  94.35 & 94.31 & \textbf{96.68} & 95.48 \\
                    & & & \textbf{94.12} & \textbf{94.89} & \textbf{95.82} & \textbf{95.34} \\
                    \multirow{-5}{*}{\textbf{VPN - ISCX}} & \multirow{-3}{*}{NetTiSA}  & \multirow{-2}{*}{KFold} & \textbf{(\(\pm\) 0.841)} & \textbf{(\(\pm\) 0.939)} & \textbf{(\(\pm\) 1.287)} & \textbf{(\(\pm\) 0.682)} \\
                    \hline
                    
                    \rowcolor{white} &   & Test  &  -- & -- & -- & 98.00  \\
                     & \multirow{-2}{*}{Jorgense et al. \cite{vnet_dataset}}   & KFold & -- & -- & -- & -- \\
                    \cline{2-7}
                    \rowcolor{white} &  &  Test & \textbf{99.98} &\textbf{100.0} & \textbf{99.44} & \textbf{99.72} \\
                    & & & \textbf{99.98}  & \textbf{99.92} &  \textbf{99.73} & \textbf{99.82} \\
                    \multirow{-5}{*}{\textbf{VPN - VNAT}} & \multirow{-3}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & \textbf{(\(\pm\) 0.015)} & \textbf{(\(\pm\) 0.273)} & \textbf{(\(\pm\) 0.418)} & \textbf{(\(\pm\) 0.224)} \\
                    \hline
                \end{tabular}
                \label{evaluation}
            \end{center}
        \end{table*}
        

==> table_multiclas_results_old.tex <==


    \subsubsection{Multi-class classification} \label{mutliclass_classification_section}
        \color{red} TODO \color{black}

        \color{red} TODO: U tabulek bychom pro setreni mistem mohli prezentovat jen Accuracy, Mactro avg., Weighted avg. a KFold -- tím redokovat výsledky ze dvou na jednu či méně A4 jak je to zde \ref{multi-class_evaluation} -- kompletní výsledky sjou zakomentovány a je možné je opět odkomentovat \color{black}


        \begin{table*}
        % \begin{minipage}{.59\linewidth}
            \caption{Final results (in \%) from the testing phase of multiclass classification based on NetTiSA flow \color{red} TODO: fill related works \color{black}}
            \begin{center}
                \begin{tabular}{|Q|Q|Y|Z{1.5cm}|Z{1.5cm}|Z{1.5cm}|Z{1.5cm}|}
                    \hline 
                    \rowcolor{Gray} \textbf{Detection problem} &  \textbf{Method} & \textbf{} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
                    \hline
                    
                     &  & Botnet & -- & 99.86  &   99.32  &   99.59 \\
                    \rowcolor{white} &  & Clear & -- & 99.63  &   98.33  &   98.97 \\
                     &  & Cryptomining & -- & 99.97  &   99.96  &   99.97 \\
                    \rowcolor{white} &  & IoT Malware & -- & 97.21  &   87.39  &   92.04 \\
                     &  &  DNS Malware & -- & 100.0  &   96.43  &  98.18 \\
                    \rowcolor{white} &  & DoH & -- &  97.32  &  99.60   & 98.44  \\
                     &  & DoS & -- & 100.0 & 100.0 & 100.0 \\
                    \rowcolor{white} &  & Tor & -- & 99.96  &  99.84   & 99.90  \\
                     &  & VPN & -- & 100.0  &  85.42   & 92.13  \\
                    \cline{3-7}
                    \rowcolor{white} &  & Macro avg. & 99.02 & 99.32  &  95.56  &  97.33 \\
                     &  & Weighted avg. &  99.02 & 99.03 & 99.02 & 99.03  \\
                    \rowcolor{white} &  &  &  99.02 & 99.03  &  99.02  &  99.02 \\
                    \rowcolor{white} \multirow{-13}{*}{\textbf{All binary together}} & \multirow{-13}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & (\(\pm\) 0.02) & (\(\pm\) 0.02) & (\(\pm\) 0.02) & (\(\pm\) 0.02) \\
                    \hline
                    \rowcolor{white}&  & Macro avg. &  &  &  &  \\
                     &  & Weighted avg. &  &  &  &  \\
                     \rowcolor{white} &  &  & -- & -- & -- & -- \\
                     \rowcolor{white} & \multirow{-4}{*}{RL \cite{}} & \multirow{-2}{*}{KFold} & \textbf{(\(\pm\) )} & \textbf{(\(\pm\) )} & \textbf{(\(\pm\) )} & \textbf{(\(\pm\) )} \\
                    \cline{2-7}
                     &  & Macro avg. & 99.72 & 79.26  &  73.87  &  76.04 \\
                    \rowcolor{white} &  & Weighted avg. & 99.72 & 99.71  &  99.72  &  99.72  \\
                     &  &  & 99.75 & 99.75  & 99.75  &  99.75  \\
                    \multirow{-8}{*}{\textbf{Botnet}} & \multirow{-4}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & (\(\pm\) 0.04) & (\(\pm\) 0.04) & (\(\pm\) 0.04) & (\(\pm\) 0.04) \\
                    \hline
                    \rowcolor{white}&  & Macro avg. &  &  &  &  \\
                     &  & Weighted avg. &  &  &  &  \\
                     \rowcolor{white} &  &  & -- & -- & -- & -- \\
                     \rowcolor{white} & \multirow{-4}{*}{RL \cite{}} &  \multirow{-2}{*}{KFold} & (\(\pm\) ) & (\(\pm\) ) & (\(\pm\) ) & (\(\pm\) ) \\
                    \cline{2-7}
                     &  & Macro avg. & 98.58 & 94.86 & 91.00 & 92.72 \\
                    \rowcolor{white} &  & Weighted avg. & 98.58 & 98.58 & 98.58 & 98.56 \\
                     &  &  & 96.04 & 96.04 & 96.04 & 96.04 \\
                    \multirow{-8}{*}{\textbf{TOR}} & \multirow{-4}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & (\(\pm\) 0.16) & (\(\pm\) 0.16) & (\(\pm\) 0.16) & (\(\pm\) 0.16) \\
                    \hline
                    \rowcolor{white} &  & Macro avg. &  &  &  &    \\
                    \rowcolor{white} & \multirow{-2}{*}{  \cite{} } &  KFold & -- & -- & -- & -- \\
                    \cline{2-7}
                     &  & Macro avg. & 94.80 & 92.12 & 90.40 & 91.21 \\
                    \rowcolor{white} &  & Weighted avg. & 94.80 &  94.76  & 94.80 & 94.77 \\
                     &  &  & 94.60 & 94.60 & 94.60 & 94.60 \\
                    \multirow{-6}{*}{\textbf{VPN - ISCX}} & \multirow{-4}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & (\(\pm\) 0.68) & (\(\pm\) 0.68) & (\(\pm\) 0.68) & (\(\pm\) 0.68) \\
                    \hline
                    \rowcolor{white}&  & Micro avg. & 96 & 96 & 96  & 96 \\
                    \rowcolor{white} & \multirow{-2}{*}{Jorgense et al.  \cite{vnet_dataset}} &  KFold & -- & -- & -- & -- \\
                    \cline{2-7}
                     &  & Macro avg. & 98.60 &  99.01  &  98.75 &  98.88 \\
                    \rowcolor{white} &  & Weighted avg. & 98.60 & 98.60  &  98.60  &  98.60 \\
                     &  &  & 99.00 & 99.00 & 99.00 & 99.00 \\
                    \multirow{-6}{*}{\textbf{VPN - VNAT}} & \multirow{-4}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & (\(\pm\) 1.10) & (\(\pm\) 1.10) & (\(\pm\) 1.10) & (\(\pm\) 1.10) \\
                    \hline
                \end{tabular}
                \label{multi-class_evaluation}
            \end{center}
        \end{table*}

        

        \begin{table*}
        % \begin{minipage}{.59\linewidth}
            \caption{Final results (in \%) from the testing phase of multiclass classification based on NetTiSA flow \color{red} TODO: fill related works \color{black}}
            \begin{center}
                \begin{tabular}{|Q|Q|Y|Z{1.5cm}|Z{1.5cm}|Z{1.5cm}|Z{1.5cm}|}
                    \hline 
                    \rowcolor{Gray} \textbf{Detection problem} &  \textbf{Method} & \textbf{} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
                    \hline
                    \rowcolor{white}&  & Macro avg. &  &  &  &  \\
                     &  & Weighted avg. &  &  &  &  \\
                     \rowcolor{white} &  &  & -- & -- & -- & -- \\
                     \rowcolor{white} & \multirow{-4}{*}{RL \cite{}} &  \multirow{-2}{*}{KFold} & (\(\pm\) ) & (\(\pm\) ) & (\(\pm\) ) & (\(\pm\) ) \\
                    \cline{2-7}
                     &  & Macro avg. & 99.83 & 75.93 & 67.25 & 70.53 \\
                    \rowcolor{white} &  & Weighted avg. & 99.83 & 99.82 & 99.83 & 99.82 \\
                     &  &  & 99.83  & 99.82 & 99.83 & 99.82 \\
                    \multirow{-8}{*}{\textbf{IDS multi-class}} & \multirow{-4}{*}{NetTiSA} & \multirow{-2}{*}{KFold} & (\(\pm\) 0.01) & (\(\pm\) 0.01) & (\(\pm\) 0.01) & (\(\pm\) 0.01) \\
                    \hline
                \end{tabular}
                \label{multi-class_evaluation_2}
            \end{center}
        \end{table*}
        
        
